Direct Distillation between Different Domains

Knowledge Distillation (KD) aims to learn a compact student network using knowledge from a large pre-trained teacher network, where both networks are trained on data from the same distribution. However, in practical applications, the student network may be required to perform in a new scenario (i.e., the target domain), which usually exhibits significant differences from the known scenario of the teacher network (i.e., the source domain). The traditional domain adaptation techniques can be integrated with KD in a two-stage process to bridge the domain gap, but the ultimate reliability of two-stage approaches tends to be limited due to the high computational consumption and the additional errors accumulated from both stages. To solve this problem, we propose a new one-stage method dubbed ``Direct Distillation between Different Domains" (4Ds). We first design a learnable adapter based on the Fourier transform to separate the domain-invariant knowledge from the domain-specific knowledge. Then, we build a fusion-activation mechanism to transfer the valuable domain-invariant knowledge to the student network, while simultaneously encouraging the adapter within the teacher network to learn the domain-specific knowledge of the target data. As a result, the teacher network can effectively transfer categorical knowledge that aligns with the target domain of the student network. Intensive experiments on various benchmark datasets demonstrate that our proposed 4Ds method successfully produces reliable student networks and outperforms state-of-the-art approaches.

==> sec/code.tex <==
\begin{algorithm}[t]
	\caption{Direct Distillation between Different Domains}
	\begin{algorithmic}[1]
		\REQUIRE Pre-trained teacher network $\mathcal{N}_{T}$ in the source domain, target data $\mathcal{D}=\left\{\left(\mathbf{x}_{i}, y_{i}\right)\right\}_{i=1}^{|\mathcal{D}|}$, trade-off parameters $\beta$ and $\gamma$.
		\STATE Initialize and integrate the learnable adapters into $\mathcal{N}_{T}$;
		\STATE Initialize the small student network $\mathcal{N}_{S}$;
		\REPEAT 
		\STATE Employ $\mathcal{N}_{S}$, $\mathcal{N}_{T}$ to obtain their predictions $\{\mathcal{N}_{S}{(\mathbf{x}_{i})}\}_{i=1}^{|\mathcal{D}|}$, $\{\mathcal{N}_{T}{(\mathbf{x}_{i})}\}_{i=1}^{|\mathcal{D}|}$, and domain-invariant features $\{\boldsymbol{\mathcal{P}}_{\text {act }, i}^S\}_{i=1}^{|\mathcal{D}|}$, $\{\boldsymbol{\mathcal{P}}_{\text {act }, i}^T\}_{i=1}^{|\mathcal{D}|}$;
		\STATE Calculate cross-entropy losses $\mathcal{L_{\mathrm{ce}}}(\mathcal{N}_{T})$ and $\mathcal{L_{\mathrm{ce}}}(\mathcal{N}_{S})$;
		\STATE Calculate knowledge transfer losses $\mathcal{L_{\mathrm{kt}}}(\mathcal{N}_{T})$ and $\mathcal{L_{\mathrm{kt}}}(\mathcal{N}_{S})$ via Eq.~(\ref{eq_ktt});
		\STATE Calculate domain-invariant knowledge transfer loss $\mathcal{L_{\mathrm{dikt}}}(\mathcal{N}_{S})$ via Eq.~(\ref{eq_dikt});
%		\STATE Calculate objective loss $\mathcal{L}_{\mathrm{total}}(\mathcal{N}_T)$ via Eq.~(\ref{eq_totalt});
		\STATE Update $\mathcal{N}_{T}$ via Adam;
%		\STATE Calculate objective loss $\mathcal{L}_{\mathrm{total}}(\mathcal{N}_S)$ via Eq.~\eqref{eq_totals};
		\STATE Update $\mathcal{N}_{S}$ via SGD;
		\UNTIL {convergence}
		\ENSURE Lightweight student network in the target domain.
	\end{algorithmic}
	\label{alg_1}
\end{algorithm}
